Automata Quest: NCAs as a Video Game Life Mechanic

We study life over the course of video game history as represented by their mechanics. While there have been some variations depending on genre or "character type", we find that most games converge to a similar representation. We also examine the development of Conway's Game of Life (one of the first zero player games) and related automata that have developed over the years. With this history in mind, we investigate the viability of one popular form of automata, namely Neural Cellular Automata, as a way to more fully express life within video game settings and innovate new game mechanics or gameplay loops.

==> reference.tex <==
@article{mordvintsev2020growing,
  author = {Mordvintsev, Alexander and Randazzo, Ettore and Niklasson, Eyvind and Levin, Michael},
  title = {Growing Neural Cellular Automata},
  journal = {Distill},
  year = {2020},
  note = {https://distill.pub/2020/growing-ca},
  doi = {10.23915/distill.00023}
}

@INPROCEEDINGS{Bjork2012-ba,
  title     = "{Zero-player games or: what we talk about when we talk about
               players}",
  booktitle = "{Philosophy of Computer Games Conference, Madrid}",
  author    = "Bj{\"o}rk, Staffan and Juul, Jesper",
  abstract  = "… by looking at zero - player games so far: that we often assume
               games to be voluntary activities (as described by Huizinga). Not
               too surprising, while zero - player games have made visible …",
  publisher = "academia.edu",
  year      =  2012,
  url       = "https://www.academia.edu/download/39691755/Zero-Player_Games_1.6___official_template.pdf",
  file      = "All Papers/B/Björk and Juul 2012 - Zero-player games or - what we talk about when we talk about players.pdf"
}


@INCOLLECTION{Horibe2021-bk,
  title     = "{Regenerating soft robots through neural cellular automata}",
  booktitle = "{Lecture Notes in Computer Science}",
  author    = "Horibe, Kazuya and Walker, Kathryn and Risi, Sebastian",
  abstract  = "This approach allows simulated soft robots that are damaged to
               partially regenerate their original morphology through local
               cell interactions alone and regain some of their ability to
               locomote. Morphological regeneration is an important feature
               that highlights the environmental adaptive capacity of
               biological systems. Lack of this regenerative capacity
               significantly limits the resilience of machines and the
               environments they can operate in. To aid in addressing this gap,
               we develop an approach for simulated soft robots to regrow parts
               of their morphology when being damaged. Although numerical
               simulations using soft robots have played an important role in
               their design, evolving soft robots with regenerative
               capabilities have so far received comparable little attention.
               Here we propose a model for soft robots that regenerate through
               a neural cellular automata. Importantly, this approach only
               relies on local cell information to regrow damaged components,
               opening interesting possibilities for physical regenerable soft
               robots in the future. Our approach allows simulated soft robots
               that are damaged to partially regenerate their original
               morphology through local cell interactions alone and regain some
               of their ability to locomote. These results take a step towards
               equipping artificial systems with regenerative capacities and
               could potentially allow for more robust operations in a variety
               of situations and environments. The code for the experiments in
               this paper is available at:
               github.com/KazuyaHoribe/RegeneratingSoftRobots.",
  publisher = "Springer International Publishing",
  pages     = "36--50",
  series    = "Lecture notes in computer science",
  year      =  2021,
  url       = "http://link.springer.com/10.1007/978-3-030-72812-0_3",
  file      = "All Papers/H/Horibe et al. 2021 - Regenerating soft robots through neural cellular automata.pdf",
  address   = "Cham",
  language  = "en",
  issn      = "0302-9743, 1611-3349",
  isbn      = "9783030728113, 9783030728120",
  doi       = "10.1007/978-3-030-72812-0\_3"
}



@book{rowlands2016video,
  title={Video Game Worlds: Working at Play in the Culture of EverQuest},
  author={Rowlands, T.},
  isbn={9781315416038},
  url={https://books.google.co.jp/books?id=YKhmDAAAQBAJ},
  year={2016},
  publisher={Taylor \& Francis}
}

@incollection{doi:10.1162/dmal.9780262693646.117,
  abstract = {Bogost's chapter offers an introduction to rhetoric in games. First he looks at the way games and their rules embody cultural values, following the work of Brian Sutton-Smith and looking in particular at a few examples from international sports. Then he discusses the relationship between games and ideology, showing how game play can unpack and expose deeply engrained social, cultural, and political assumptions. Finally he discusses the ways videogames make arguments. Drawing on the history of rhetoric, Bogost introduces a notion he calls “procedural rhetoric,” the art of persuasion through rule-based representations and interactions.},
  added-at = {2010-09-16T18:58:56.000+0200},
  author = {Bogost, Ian},
  biburl = {https://www.bibsonomy.org/bibtex/2116f2ceb10a8a787aacdcacd36e7ad04/yish},
  booktitle = {The Ecology of Games: Connecting Youth, Games, and Learning},
  doi = {10.1162/dmal.9780262693646.117},
  eprint = {http://www.mitpressjournals.org/doi/pdf/10.1162/dmal.9780262693646.117},
  interhash = {52dcad968af9e386291fc8ea8e220908},
  intrahash = {116f2ceb10a8a787aacdcacd36e7ad04},
  journal = {The John D. and Catherine T. MacArthur Foundation Series on Digital Media and Learning},
  keywords = {education games haifa-games-course learning},
  pages = {117-139},
  publisher = {The John D. and Catherine T. MacArthur Foundation Series on Digital Media and Learning},
  timestamp = {2010-09-16T18:58:56.000+0200},
  title = {The Rhetoric of Video Games},
  url = {http://www.mitpressjournals.org/doi/abs/10.1162/dmal.9780262693646.117},
  year = 2007
}


@article{doi:10.1177/1555412014557542,
author = {Sun-ha Hong},
title ={When Life Mattered: The Politics of the Real in Video Games’ Reappropriation of History, Myth, and Ritual},
journal = {Games and Culture},
volume = {10},
number = {1},
pages = {35-56},
year = {2015},
doi = {10.1177/1555412014557542},

URL = { 
        https://doi.org/10.1177/1555412014557542
    
},
eprint = { 
        https://doi.org/10.1177/1555412014557542
}
,
    abstract = { Games borrow ceaselessly from the past to constitute themselves. This locates the medium at the heart of our contemporary obsession with how to engage the past and the “real.” In tethering digital hyperreality to the horizon of history, myth, and ritual, games generate a disavowed and subjunctive engagement with a sense of “real enough.” They thus resemble Victor Turner’s liminoids: autotelic, bounded experiences of leisure that cultivate accepting yet playful attitudes against the “real enough” on offer. This commercialized bricolage is not dismissible as inauthentic simulacrum. Rather, such games demonstrate the ways in which new media are recalibrating our modes of engagement with the real. This article analyzes three key aspects of liminoid games: (1) techniques of reappropriation during production, (2) rules and expectations of engagement with the past and the “real” that games offer, and (3) emergent ways in which player communities, discourses, and productions recalibrate those politics of engagement. }
}

@article{315e6dd32071450baefd68546019f80c,
title = "Survival horrality: analysis of a videogame genre",
abstract = "This article explores the {\textquoteleft}survival horror{\textquoteright} videogame – a genre including such series as Resident Evil, Silent Hill, Clock Tower, Fatal Frame and Forbidden Siren. The title is drawn from Philip Brophy{\textquoteright}s 1983 essay which coins the neologism {\textquoteleft}horrality{\textquoteright}, a merging of horror, textuality, morality and hilarity. Like Brophy{\textquoteright}s original did of 1980s horror cinema, this article examines characteristics of survival horror videogame text, and seeks to illustrate the relationship between {\textquoteleft}new{\textquoteright} (media) horror and {\textquoteleft}old{\textquoteright} (media) horror. Brophy{\textquoteright}s term structures this investigation around key issues and aspects of survival horror videogames. Horror relates to generic parallels with similarly-labelled film and literature, including gothic fiction, American horror cinema and traditional Japanese culture. Textuality examines the aesthetic qualities of survival horror, including the games{\textquoteright} use of narrative, their visual design and structuring of virtual spaces. Morality explores the genre{\textquoteright}s ideological characteristics, the nature of survival horror violence, the familial politics of these texts, and their reflection on issues of institutional and bodily control. Hilarity refers to moments of humour and postmodern self reflexivity, leading to consideration of survival horror{\textquoteright}s preoccupation with issues of vision, identification, and the nature of the videogame medium.",
author = "Ewan Kirkland",
year = "2011",
month = oct,
language = "English",
volume = "10",
journal = "The Irish Journal of Gothic and Horror Studies",
issn = "2009-0374",
}

% これ参考に
@software{wow,
    title={World of Warcraft},
    author={{Blizzard Entertainment: Irvine}},
    publisher={{Blizzard Entertainment: Irvine}},
    howpublished = "PC [Game]",
    year = {2004},
}

@book{sutton2018reinforcement,
  title={Reinforcement learning: An introduction},
  author={Sutton, Richard S and Barto, Andrew G},
  year={2018},
  publisher={MIT press}
}

@book{9780880387293,
  Author = {Gary Gygax and David Cook},
  Title = {The Dungeon Master Guide, No. 2100, 2nd Edition (Advanced Dungeons and Dragons)},
  Publisher = {TSR, Inc},
  Year = {1989},
  ISBN = {0880387297},
  URL = {https://www.amazon.com/Dungeon-Master-Advanced-Dungeons-Dragons/dp/0880387297?SubscriptionId=AKIAIOBINVZYXZQZ2U3A&tag=chimbori05-20&linkCode=xm2&camp=2025&creative=165953&creativeASIN=0880387297}
}

@software{darkestdungeon,
    title={{Darkest Dungeon}},
    author={{Red Hook Studios: Vancouver}},
    publisher={{Red Hook Studios: Vancouver}},
    howpublished="PC [Game]",
    year={2016},
}

@software{pokemon,
    title={{Pocket Monsters Red and Green}},
    author={{Nintendo: Kyoto}},
    publisher={{Nintendo: Kyoto}},
    howpublished="Game Boy [Game]",
    year={1996},
}

@software{darksouls,
    title={{Dark Souls}},
    author={{Namco Bandai: Tokyo}},
    publisher={{Namco Bandai: Tokyo}},
    howpublished="PC [Game]",
    year={2011},
}

@software{fallout,
    title={{Fallout 4}},
    author={{Bethesda Softworks: Maryland}},
    publisher={{Bethesda Softworks: Maryland}},
    howpublished="PC [Game]",
    year={2015},
}

@software{monsterhunter,
    title={{Monster Hunter}},
    author={{Capcom: Osaka}},
    publisher={{Capcom: Osaka}},
    howpublished="PS2 [Game]",
    year={2004},
}

@software{skyrim,
    title={{The Elder Scrolls V: Skyrim}},
    author={{Bethesda Softworks: Maryland}},
    publisher={{Bethesda Softworks: Maryland}},
    howpublished="PC [Game]",
    year={2011},
}

@software{masseffect,
    title={{Mass Effect 2}},
    author={{Electronic Arts: Redwood City}},
    publisher={{Electronic Arts: Redwood City}},
    howpublished="Xbox 360 [Game]",
    year={2010},
}

@software{amnesia,
    title={{Amnesia: The Dark Descent}},
    author={{Frictional Games: Malmö}},
    publisher={{Frictional Games: Malmö}},
    howpublished="PC [Game]",
    year={2010},
}

@software{dow,
    title={{Warhammer 40,000: Dawn of War}},
    author={{THQ: Agoura Hills}},
    publisher={{THQ: Agoura Hills}},
    howpublished="PC [Game]",
    year={2004},
}

@software{left4dead,
    title={{Left 4 Dead 2}},
    author={{Valve Corporation: Bellevue}},
    publisher={{Valve Corporation: Bellevue}},
    howpublished="PC [Game]",
    year={2009},
}

@software{minecraft,
    title={{Minecraft}},
    author={{Mojang Studios: Stockholm}},
    publisher={{Mojang Studios: Stockholm}},
    howpublished="PC [Game]",
    year={2011},
}


@software{smb,
    title={{Super Mario Bros.}},
    author={{Nintendo: Kyoto}},
    publisher={{Nintendo: Kyoto}},
    howpublished = "Famicom [Game]",
    year = {1985},
}



@incollection{tropism,
        Author={Britannica, The Editors of Encyclopedia},
        Title={Tropism},
        Year={2023},
        Booktitle={Encyclopedia Britannica}
}

@book{Wolfram2002,
    Author = {Wolfram, Stephen},
    Title = {A New Kind of Science},
    Year = {2002},
    Publisher = {Wolfram Media},
    pages = {876},
    ISBN = {1579550088},
    URL = {https://www.wolframscience.com},
    Language = {English}
    }

@InProceedings{voxel,
author="Roper, Mark
and Katsaros, Nikolaos
and Fernando, Chrisantha",
editor="del Pobil, Angel P.
and Chinellato, Eris
and Martinez-Martin, Ester
and Hallam, John
and Cervera, Enric
and Morales, Antonio",
title="Voxel Robot: A Pneumatic Robot with Deformable Morphology",
booktitle="From Animals to Animats 13",
year="2014",
publisher="Springer International Publishing",
address="Cham",
pages="230--239",
abstract="The Voxbot is a cubic (voxel) shaped robot actuated by expansion and contraction of its 12 edges designed for running evolutionary experiments, built as cheaply as possible. Each edge was made of a single 10ml medical syringe for pneumatic control. These were connected to an array of 12 servos situated on an external housing and controlled with an Arduino microcontroller from a laptop. With twenty motor primitive commands and the slow response of its pneumatics this robot allows real time controllers to be evolved in situ rather than just in simulation. With simple combinations and sequencing of motor primitives the Voxbot can be made to walk, rotate and crab crawl. The device is available in kit form and is very easy to build and replicate. Other morphologies can be built easily.",
isbn="978-3-319-08864-8"
}
